A Unified One-Step Solution for Aspect Sentiment Quad Prediction

Aspect sentiment quad prediction (ASQP) is a challenging yet significant subtask in aspect-based sentiment analysis as it provides a complete aspect-level sentiment structure. However, existing ASQP datasets are usually small and low-density, hindering technical advancement. To expand the capacity, in this paper, we release two new datasets for ASQP, which contain the following characteristics: larger size, more words per sample, and higher density. With such datasets, we unveil the shortcomings of existing strong ASQP baselines and therefore propose a unified one-step solution for ASQP, namely One-ASQP, to detect the aspect categories and to identify the aspect-opinion-sentiment (AOS) triplets simultaneously. Our One-ASQP holds several unique advantages: (1) by separating ASQP into two subtasks and solving them independently and simultaneously, we can avoid error propagation in pipeline-based methods and overcome slow training and inference in generation-based methods; (2) by introducing sentiment-specific horns tagging schema in a token-pair-based two-dimensional matrix, we can exploit deeper interactions between sentiment elements and efficiently decode the AOS triplets; (3) we design ``[NULL]'' token can help us effectively identify the implicit aspects or opinions. Experiments on two benchmark datasets and our released two datasets demonstrate the advantages of our One-ASQP. The two new datasets are publicly released at \url{https://www.github.com/Datastory-CN/ASQP-Datasets}.

==> App20230119.tex <==
\appendix

\section{More Details about Datasets Construction}\label{app:datasets}
This section provides more details about constructing the two released datasets, en-Phone and cn-FoodBeverage. % , xxx, including the definition of aspect categories and annotation guidelines, of

\subsection{Data Sources}\label{app:source}
The English ASQP dataset, en-Phone, is collected from reviews on Amazon UK~\footnote{\url{https://www.amazon.co.uk/}}, Amazon India~\footnote{\url{https://www.amazon.in/}} and Shopee~\footnote{\url{https://shopee.com.my/}} in July and August of 2021, covering 12 cell phone brands, such as Samsung, Apple, Huawei, OPPO, Xiaomi, etc.  

The first Chinese ASQP dataset, cn-FoodBeverage, is collected from the Chinese comments on  forums~\footnote{\url{http://foodmate.net/}}, Weibo~\footnote{\url{https://weibo.com/}}, news~\footnote{\url{https://chihe.sohu.com/}} and e-commerce platforms~\footnote{\url{https://www.jd.com/},\url{https://www.taobao.com/}} in the years 2019-2021 under the categories of Food and Beverage.

%
%The category is two layers, distinguished by ``\#''. Such as ``Screen\#Sensitivity'' in en\#Phone, ``Screen'' belongs to the first level dimension, ``Sensitivity'' belongs to the second level dimension under ``Screen''.

% category类别
%The numbers of categories for en-Phone and cn-FoodBeverage were 64, 116, respectively. For each category we have more than 20 quadruple labeled. Compare to Laptop-ACOS, although there are 121 categories, filtering out the categories with less than 20 annotations, only 45 remain.


\subsection{Annotation Guidelines}\label{app:guideline}

% 大部分的标注规范
%This task requires the annotators to label four parts in the corpus, including aspect, category, opinion and sentiment, and combine them as a whole quadruple.  a unique predefined category for the aspect in a particular domain Some examples with aspect and category pairs are shown as follows.

The following outlines the guidelines for annotating the four fundamental sentiment elements of ASQP, i.e., aspect categories, aspect terms, opinion terms, and sentiment polarity, and the outcomes.  It can be noted that our labeled ASQP quadruples are more fine-grained and more difficult than those in existing ASQP benchmark datasets. 

\subsubsection{Aspect Categories}\label{app:categories}
The aspect categories are two-level categories defined by business experts in the related field.  As the example shown in Fig.~\ref{fig:model}, a category is ``Screen\#Sensitivity'', where ``Screen'' is the first-level category and ``Sensitivity'' is the second-level category, which specifies an attribute of the ``Screen''.   \blue{In our experiments, we only consider the second-level categories.  }

As reported in Table~\ref{tab:datasets}, the number of categories for en-Phone and cn-FoodBeverage is 64 and 116, respectively.  The number of labeled quadruples per category is larger than 20.  Though Laptop-ACOS consists of 121 categories, if we filter out the categories with less than 20 annotated quadruples, the number of categories is reduced to 45.  Hence, we provide more dense and rich datasets for ASQP. 
%.  It can be seen that our annotation is followed the need for real-world commercial applications. 
 %It is more fine-grained and more difficult than existing ASQP benchmark datasets.
\begin{compactitem}
\item The \textbf{aspect category} defines the type of the concerned aspect.  As described in Sec.~\ref{app:categories}, we define the aspect categories in two-level, which provide more detailed information for the need of commercial applications.  Here, we list some typical examples of the aspect category for the opinionated sentence: 
\begin{compactitem}
\item ``{Security\#Screen Unlock}'': Don't like face recognition and battery life. %(\textcolor{category}{Security\#Screen Unlock}, \textcolor{aspect}{face recognition})(\textcolor{category}{Battery/Longevity\#Battery life}, \textcolor{aspect}{battery life})
\item ``Price\#General'': It's very cheap. First time I bought the phone I wanted. %(\textcolor{category}{Price\#General}, \textcolor{aspect}{cheap})
\item \blue{``Logistics\#Speed'' and ``Overall Rating\#General'': Very fast delivery \& phone is working well}
\end{compactitem}
%\paragraph{Aspect} 
\item The \textbf{aspect} term is usually a noun or a noun phrase, indicating the opinion target, in the text.   However, in our annotation guideline, we include three additional rules: 
\begin{enumerate}[(1)]
    \item The aspect term can be an adjective when it holds the sentiment orientation.  For example, as the example of en-Phone in Table~\ref{tab:ex_illustration}, ``recommended'' is also labeled as an aspect in the opinionated sentence, ``Highly recommended''.  ``cheap'' is labeled as the aspect term in the above example of ``It's very cheap. First time I bought the phone I wanted.''
    \item Pronoun is not allowed to be an aspect term as it cannot be identified by the quadruples.  For example, in the sentence ``pretttyyyy and affordable too!!! I love it!!  Thankyouuu!!'', ``it'' cannot be labeled as the aspect though we know it means a phone from the context.  
    \item Top-priority in labeling fine-grained aspects.  For example, \red{xxx}.  % 优先标维度更细的特征词
\end{enumerate}
\item The \textbf{opinion} term describes the sentiment towards the aspect.  \blue{An opinion term is usually an adjective or a phrase with sentiment polarity. }  Here, we include more labeling rules:
\begin{enumerate}[(1)]
    \item When there is a negative word, e.g., ``Don't'', ``NO'', ``cannot'', ``doesn't'', the negative word should be included in the opinion term.  For example, ``Don’t like'' is the opinion term in ``\textcolor{opinion}{Don’t like} face recognition and battery life.''
    \item Where there is an adverb or a preposition, e.g., ``very'', ``too'', ``so'', ``inside'', ``under'', ``outside'', the corresponding adverb or preposition should be included in the opinion term.  For example, ``very cheap'' is the opinion term in ``It's \textcolor{opinion}{very cheap}. The first time I bought the phone I wanted.''.  Meanwhile, ``Very fast'' and ``working well'' are the corresponding opinion terms in ``\textcolor{opinion}{Very fast} delivery \& phone is \textcolor{opinion}{working well}''.
\end{enumerate}
\item The \textbf{sentiment polarity} belongs to one of the sentiment classes, \{POS, NEU, NEG\}, for the positive, neutral, and negative sentiment, respectively.  We present several examples and ASQP quadruples in Table~\ref{tab:ex_quadruples}: 
\end{compactitem}

\begin{table*}[]
\small
\centering
    \begin{tabular}{l@{~}l@{~~}c}
    \hline
    &\multicolumn{1}{c}{Sentence} & Labeled Quadruples \\\hline
    %\begin{minipage}{5.4cm}
    %    \begin{tabular}{p{5.4cm}}
    Ex.~1 & \textcolor{opinion}{Don’t like} \textcolor{aspect}{face recognition} and \textcolor{aspect}{battery life}.
    %\end{tabular}
    %\end{minipage}
    & 
    \begin{minipage}{8cm}
        \begin{tabular}{p{8cm}}
            (\textcolor{category}{Security\#Screen Unlock}, \textcolor{aspect}{face recognition}, \textcolor{opinion}{Don’t like}, \textcolor{sentiment}{NEG})\\
            (\textcolor{category}{Battery/Longevity\#Battery life}, \textcolor{aspect}{battery life}, \textcolor{opinion}{Don't like}, \textcolor{sentiment}{NEG})
        \end{tabular}
    \end{minipage}\\\hline
    %\begin{minipage}{5.4cm}
    %    \begin{tabular}{p{5.4cm}}
   Ex.~2 &   \textcolor{opinion}{Very fast} \textcolor{aspect}{delivery} \& \textcolor{aspect}{phone} is \textcolor{opinion}{working well}.        
    % \end{tabular}
    %\end{minipage} 
    & 
      \begin{minipage}{8.cm}
        \begin{tabular}{p{8.cm}}
        (\textcolor{category}{Logistics\#Speed}, \textcolor{aspect}{delivery}, \textcolor{opinion}{Very fast}, \textcolor{sentiment}{POS})\\
        (\textcolor{category}{Overall Rating\#General}, \textcolor{aspect}{phone}, \textcolor{opinion}{working well}, \textcolor{sentiment}{POS})
      \end{tabular}
    \end{minipage}
      \\\hline
    Ex.~3 &  \begin{minipage}{6.5cm}
        \begin{tabular}{@{~}p{7cm}}
       It's very \textcolor{aspect}{cheap}.  The first time I bought the phone I wanted. 
       \end{tabular}
    \end{minipage}
    & 
      \begin{minipage}{8.cm}
        \begin{tabular}{p{8.cm}}
       (\textcolor{category}{Price\#General}, \textcolor{aspect}{cheap}, \textcolor{opinion}{NULL}, \textcolor{sentiment}{POS})
       \end{tabular}
    \end{minipage}
       \\\hline
    \end{tabular}
    \caption{Three opinionated sentences and the labeled quadruples.  }
    \label{tab:ex_quadruples}
\end{table*}
\if 0
\begin{table*}[]
\small
\centering
    \begin{tabular}{@{~}l@{~~}c}
    \hline
    \multicolumn{1}{c}{Sentence} & Labeled Quadruples \\\hline
    %\begin{minipage}{5.4cm}
    %    \begin{tabular}{p{5.4cm}}
    \textcolor{opinion}{Don’t like} \textcolor{aspect}{face recognition} and \textcolor{aspect}{battery life}.
    %\end{tabular}
    %\end{minipage}
    & 
    \begin{minipage}{8.cm}
        \begin{tabular}{p{8.cm}}
            (\textcolor{category}{Security\#Screen Unlock}, \textcolor{aspect}{face recognition}, \textcolor{opinion}{Don’t like}, \textcolor{sentiment}{NEG})\\
            (\textcolor{category}{Battery/Longevity\#Battery life}, \textcolor{aspect}{battery life}, \textcolor{opinion}{Don't like}, \textcolor{sentiment}{NEG})
        \end{tabular}
    \end{minipage}\\\hline
    %\begin{minipage}{5.4cm}
    %    \begin{tabular}{p{5.4cm}}
      \textcolor{opinion}{Very fast} \textcolor{aspect}{delivery} \& \textcolor{aspect}{phone} is \textcolor{opinion}{working well}.        
    % \end{tabular}
    %\end{minipage} 
    & 
      \begin{minipage}{8.cm}
        \begin{tabular}{p{8.cm}}
        (\textcolor{category}{Logistics\#Speed}, \textcolor{aspect}{delivery}, \textcolor{opinion}{Very fast}, \textcolor{sentiment}{POS})\\
        (\textcolor{category}{Overall Rating\#General}, \textcolor{aspect}{phone}, \textcolor{opinion}{working well}, \textcolor{sentiment}{POS})
      \end{tabular}
    \end{minipage}
      \\\hline
      \begin{minipage}{5.4cm}
        \begin{tabular}{@{~}l}
       It's very \textcolor{aspect}{cheap}.  The first time I bought the phone I wanted. 
       \end{tabular}
    \end{minipage}
    & 
      \begin{minipage}{8.cm}
        \begin{tabular}{p{8.cm}}
       (\textcolor{category}{Price\#General}, \textcolor{aspect}{cheap}, \textcolor{opinion}{NULL}, \textcolor{sentiment}{POS})
       \end{tabular}
    \end{minipage}
       \\\hline
    \end{tabular}
    \caption{Three opinionated sentences and the labeled quadruples.  }
    \label{tab:ex_quadruples}
\end{table*}
\fi 
\if 0
positive, neutral, and negative. Some examples with ASQP quadruples are shown as follows.
\begin{compactitem}
\item Don’t like face recognition and battery life. $\Rightarrow$(\textcolor{category}{Security\#Screen Unlock}, \textcolor{aspect}{face recognition}, \textcolor{opinion}{Don’t like}, \textcolor{sentiment}{NEG}) , (\textcolor{category}{Battery/Longevity\#Battery life}, \textcolor{aspect}{battery life}, \textcolor{opinion}{Don't like}, \textcolor{sentiment}{NEG})
\item Very fast delivery \& phone is working well. $\Rightarrow$(\textcolor{category}{Logistics\#Speed}, \textcolor{aspect}{delivery}, \textcolor{opinion}{Very fast}, \textcolor{sentiment}{POS}), (\textcolor{category}{Overall Rating\#General}, \textcolor{aspect}{phone}, \textcolor{opinion}{working well}, \textcolor{sentiment}{POS})
\item It's very cheap, First time I bought the phone I wanted. $\Rightarrow$(\textcolor{category}{Price\#General}, \textcolor{aspect}{cheap}, \textcolor{opinion}{null}, \textcolor{sentiment}{POS})
\end{compactitem}



\red{When the aspect itself there is sentiment, and there is an adverb / negative word to modify the aspect term, the adverb / negative word is labeled as opinion.  Opinion is usually an adjective or or phrases with sentiment polarity, when there is a negative word/adverb, the negative word/adverb should be included in the opinion.}  \blue{fine-grained }

In the following, we highlight the corresponding opinion terms, including ``don’t like '', ``very cheap'', ``Very fast'' and ``working well'' are opinions.
\begin{compactitem}
\item \textcolor{opinion}{Don’t like} face recognition and battery life.
\item \red{It's very cheap. First time I bought the phone I wanted.}
\item \textcolor{opinion}{Very fast} delivery \& phone is \textcolor{opinion}{working well}.
\end{compactitem}
When the feature word itself has emotion and there is an adverb/negative modifying the feature word, the adverb/negative is marked as an emotion word, when the role of the emotion word is to aggravate the degree of emotion/determine the final emotion.
\begin{compactitem}
\item It's \textcolor{opinion}{very} cheap, First time I bought the phone I wanted.
\end{compactitem}

modifying the aspect term with the opinion term can determine the sentiment polarity. 

\fi 



% while the corresponding category is ``Buyer attitude#Recommendable''.

%For example, in Table~\ref{tab:ex_illustration}, ``lactoferrin'', ``, baby absorption'',  

%the category of the annotation content can be determined by the aspect term alone, the aspect is usually a noun or noun phrase. In the following example, ``face recognition'', ``battery life'', ``delivery'' and ``phone'' are aspects.

\if 0
\begin{compactitem}
\item Don't like the \textcolor{aspect}{face recognition} and \textcolor{aspect}{battery life}. 
\item Very fast \textcolor{aspect}{delivery} \& \textcolor{aspect}{phone} is working well. 
\end{compactitem}

the aspect may be an adjective when the aspect term itself has an emotional orientation. In the following example, ``cheap'' is aspect, because through it we know that the buyer wants to comment on the Price\#General category. 
\begin{compactitem}
\item It's very \textcolor{aspect}{cheap}, First time I bought the phone I wanted.
\end{compactitem}
\fi 




\red{
\subsection{Details}\label{app:details} 
For example, given an example, ``five stars with no doubt'', we will label ``no doubt'' as an opinion while Restaurant-ACOS and Laptop-ACOS will not.  For another example of ``very good'', we will label all as its opinion while Restaurant-ACOS and Laptop-ACOS only label the word ``good'' as the opinion.

\paragraph{Explicit Aspect \& Implicit Opinion} Due to our annotation specification, an aspect term can exist without a corresponding opinion when this aspect can determine both category and sentiment. There can be no opinions in the quadruple, but there must be an explicit aspect, so we only label the implicit opinion and not the implicit aspects. As in the example below, by using word ``good'' and contextual semantics, we can know that the buyer is commenting on the Overall Rating\#General category, so mark ``good'' as aspect, where there is no explicit opinion. 
\begin{compactitem}
\item Good, I've been using it for three months. $\Rightarrow$(\textcolor{category}{Security\#Screen Unlock}, \textcolor{aspect}{face recognition}, \textcolor{opinion}{Don’t like}, \textcolor{sentiment}{NEG}) , (\textcolor{category}{Battery/Longevity\#Battery life}, \textcolor{aspect}{battery life}, \textcolor{opinion}{Don't like}, \textcolor{sentiment}{NEG})
\end{compactitem}
}
% \red{
% Example
% \begin{quote}
% Iphone 14 pro max = No sound game sound. Fix it please. \#\#\#\#[['23,28', 'Software Performance:Audio Performance', '0', '20,22']]
% \end{quote}
% Each line consists of review text and its quadruples. Each quadruple is formalized as `Aspect Category Sentiment Opinion'. The 0, 1, 2 in the Sentiment category represents negative, neutral, and positive, respectively.
% }


In Table~\ref{fig:ex_illustration}, we show examples with longer sentences and a larger number of quadruples.  

\begin{CJK*}{UTF8}{gbsn}
\begin{table*}[htpb]
\small
\centering%\footnotesize
\begin{tabular}%{@{~~~~}l@{~~~~}l@{~~~~}l@{~~~~}}
{@{~}l@{~}c@{~~}c%p{7.5cm}
}
\hline
Source & Opinionated sentences & Quadruples \\\hline
%\multirow{1}{*}
% {en-Phone\\} 
{en-Phone} 
&  
\begin{minipage}{4.4cm}
\begin{tabular}{p{4.4cm}}
{Item received took a long time. Looks nice and good quality too. Price is cheaper than retail costs. Bought it for my mom and she likes it! Highly recommended.} \\\\
\end{tabular}
 \end{minipage}
 & 
\begin{minipage}{8.cm}
\begin{tabular}{p{8.cm}}
    (\textcolor{category}{Logistics\#Logistics speed}, \textcolor{aspect}{Item received}, \textcolor{opinion}{took a long time}, \textcolor{sentiment}{NEG}), \\
 (\textcolor{category}{Exterior Design\#Aesthetics}, \textcolor{aspect}{Looks}, \textcolor{opinion}{nice}, \textcolor{sentiment}{POS}), \\
  (\textcolor{category}{Product Quality\#General}, \textcolor{aspect}{quality}, \textcolor{opinion}{good}, \textcolor{sentiment}{POS}), \\
(\textcolor{category}{Price\#General}, \textcolor{aspect}{Price}, \textcolor{opinion}{heaper than retail costs}, \textcolor{sentiment}{POS}), \\
  (\textcolor{category}{Audience\#Users}, \textcolor{aspect}{mom}, \textcolor{opinion}{likes}, \textcolor{sentiment}{POS}), \\
 (\textcolor{category}{Buyer attitude\#Recommendable}, \textcolor{aspect}{recommended}, \textcolor{opinion}{Highly likes}, \textcolor{sentiment}{POS})
 \end{tabular}
 \end{minipage}
\\ \hline
%PHED$_{\rm \mathbf{H}\underline{I}}$ & {\bf 哈哈}，\underline{米兰这是要逆天吗？} %& 
%\\&{\bf Haha}, \underline{is Milan going to offence God's will?} \\
{\multirow{1}{*}{cn-FoodBeverage}} & 
\begin{minipage}{4.4cm}
\begin{tabular}{p{4.4cm}}
我挑选这个品牌的主要原因是它这里含一项乳铁蛋白促进宝宝吸收的，所以宝宝喝它没有奶瓣的情况，同时它的口味也接近母乳，宝宝很爱喝。可惜的是，买了那么多奶粉，赠品没收到，也不知道哪个环节出的问题，连赠品的影子都没看见，只能认倒霉了，无处对证去%& 
\\  The main reason I picked this brand is that it contains Lactoferrin to promote baby's absorption, so the baby drinks it without a milk valve, while its taste is also close to breast milk, the baby loves to drink.  Unfortunately, I bought so much milk powder and did not receive a gift, and I do not know which part of the problem, even the shadow of the gift did not see, can only admit bad luck, there is no evidence to testify. 

%In the case of a baby drinking it without a milk valve, At the same time, its taste is close to that of breast milk, babyBao likes to drink very much. Unfortunately, I bought that There are so many milk powders, the gift has not been received, nor If you know which link is the problem, please donate I didn't even see the shadow of the product, I could only recognize it Moldy, nowhere to testify

%The main reason for this brand is that it contains a lactoferrin to promote baby absorption, so the baby drinks it without milk flaps, while its taste is also close to breast milk, the baby loves to drink. Unfortunately, buy so much milk powder, the gift did not receive, and I do not know which part of the problem, even the shadow of the gift did not see, can only admit bad luck, there is no evidence to go.  
\end{tabular}
 \end{minipage} 
 & 
 \begin{minipage}{8.cm}
\begin{tabular}{p{8.cm}}
    (\textcolor{category}{成分\#营养成分}, \textcolor{aspect}{乳铁蛋白}, \textcolor{opinion}{含}, \textcolor{sentiment}{POS}), \\     
    (\textcolor{category}{营养\#吸收}, \textcolor{aspect}{宝宝吸收}, \textcolor{opinion}{促进}, \textcolor{sentiment}{POS}), \\
    (\textcolor{category}{不良反应\#其他不适}, \textcolor{aspect}{奶瓣}, \textcolor{opinion}{没有}, \textcolor{sentiment}{POS}), \\
    (\textcolor{category}{味道\#综合味道}, \textcolor{aspect}{口味}, \textcolor{opinion}{接近母乳}, \textcolor{sentiment}{POS}), \\
    (\textcolor{category}{使用\#受众群体}, \textcolor{aspect}{宝宝}, \textcolor{opinion}{爱喝}, \textcolor{sentiment}{POS}), \\
    (\textcolor{category}{促销\#赠品}, \textcolor{aspect}{赠品}, \textcolor{opinion}{没收到}, \textcolor{sentiment}{NEG}), \\
    (\textcolor{category}{促销\#赠品}, \textcolor{aspect}{赠品}, \textcolor{opinion}{没看见}, \textcolor{sentiment}{NEG}), \\
 \\
 \\
     (\textcolor{category}{Ingredients\#Nutritional Composition}, \textcolor{aspect}{lactoferrin}, \textcolor{opinion}{contains}, \textcolor{sentiment}{POS}), \\
     (\textcolor{category}{Nutrition\#Absorption}, \textcolor{aspect}{baby's absorption}, \textcolor{opinion}{promote}, \textcolor{sentiment}{POS}), \\
     (\textcolor{category}{Adverse reactions\#Other discomfort}, \textcolor{aspect}{milk valve}, \textcolor{opinion}{without}, \textcolor{sentiment}{POS}), \\
     (\textcolor{category}{Flavor\#Comprehensive flavor}, \textcolor{aspect}{taste}, \textcolor{opinion}{close to breast milk}, \textcolor{sentiment}{POS}), \\
     (\textcolor{category}{Use\#Audience group}, \textcolor{aspect}{baby}, \textcolor{opinion}{loves to drink}, \textcolor{sentiment}{POS}), \\
     (\textcolor{category}{Promotion\#Giveaway}, \textcolor{aspect}{gift}, \textcolor{opinion}{did not receive}, \textcolor{sentiment}{NEG}), \\
     (\textcolor{category}{Promotion\#Giveaway}, \textcolor{aspect}{gift}, \textcolor{opinion}{did not see}, \textcolor{sentiment}{NEG}), \\

 \end{tabular}
 \end{minipage}
\\ \hline
% {\multirow{1}{*}{Quadruple}} & XXXX %& 
% \\ & XXXX \\ \hline
\end{tabular}
\caption{Typical examples of the labeled quadruples in en-Phone and cn-FoodBeverage.
\label{tab:ex_illustration}}
\end{table*}
\end{CJK*}

\subsection{Quaternion density for different datasets}\label{app:quads_density}
\blue{
\begin{CJK*}{UTF8}{gbsn}
\begin{figure}[ht] 
\centering 
\includegraphics[scale=0.06]{./pic/quads_num.png}
\caption{} 
\label{fig:quads_num} 
\end{figure}

从Fig.~\ref{fig:quads_num}可以看到，Restaurant-ACOS和Laptop-ACOS，样本有0个或1个的四元组比例高达61.12\%和71.54\%，而本文提出的en-Phone和cn-FoodBeverage只有39.33\%和39.10\%，en-Phone和cn-FoodBeverage拥有三个及三个三元组的比例为35.19\%和34.01\%，反观Restaurant-ACOS和Laptop-ACOS只有14.09\%和8.34\%，因此，新的数据集有更密集的四元组密度。
\end{CJK*}
}

\subsection{Computational Efficiency}\label{app:efficiency}
\blue{
\begin{CJK*}{UTF8}{gbsn}

如 Table~\ref{tab:all_time}所示，为所有模型的耗费时间，可以看到OneASQP在训练和推理效率是都是最佳的。

\begin{table*}[]
\small
\centering
\begin{tabular}{l@{~}|c@{~}c@{~}|c@{~}c@{~}|c@{~}c@{~}|c@{~}c@{~}}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Restaurant-ACOS}} & \multicolumn{2}{c|}{\textbf{Laptop-ACOS}} & \multicolumn{2}{c|}{\textbf{en-Phone}} & \multicolumn{2}{c}{\textbf{cn-FoodBeverage}}\\ \cline{2-9} 
& {{Train}} & {{Inference}} & {{Train}} & {{Inference}} & {{Train}} & {{Inference}} & {{Train}} & {{Inference}} \\ \hline
Extract-Classify & 38.43 & 32.23 & 72.25 & 20.23 & 158.34 & 25.23 & 301.42 & 70.34 \\
Paraphrase & 48.23 & 53.75 & 71.43 & 92.35 & 202.32 & 150.56 & 350.56 & 303.25 \\ \hline
OneASQP (base) & 11.23 & 6.34 (29.35) & 19.03 & 8.34 (39.83) & 32.23 & 6.32 (35.45) & 71.23 & 13.23 (31.74) \\
OneASQP (large) & 17.63 & 14.63 (44.62) & 36.63 & 8.45 (49.45) & 105.23 & 10.34 (61.23) & 140.23 & 30.46 (56.32) \\ 
\hline
\end{tabular}
\caption{Time cost in seconds on Restaurant-ACOS and en-Phone.  For fair comparison with baselines, we record our One-ASQP  inference time when setting the batch size to 1 and report them in the round bracket.  The default batch size is 32. }
\label{tab:all_time}
\end{table*}

\end{CJK*}
}

\subsection{Effect of Variants of Interactions}
\blue{
\begin{CJK*}{UTF8}{gbsn}
为了验证我们把ASQP拆分成ACD和AOSC两个子任务的合理性，这里提出OneASQP的两个变种

\paragraph{变种1}把ASQP拆分成aspect-opinion pair对的识别、aspect category序列识别、sentiment序列识别三个子任务。具体的，我们把Sec.~\ref{sec:ASOC}的AB-OE-*SENTIMENT标签变成AB-EO，这样原来的tag空间从5个变成只有\{AB-OB, AE-OE, AB-OE\} 3个，二维矩阵只用来抽取有关联的aspect和opinion对，sentiment的识别用另外一条序列进行预测。
\paragraph{变种2}把ASQP建模成一个任务。具体的，我们也是在标签上做文章，我们把Sec.~\ref{sec:ASOC}的AB-EO-*SENTIMENT标签扩展为AB-OE-*SENTIMENT-*CATEGORY，这样原来的tag空间从5个变成$2+|\gS|*|\gC|$($|\gS|$为sentiment的类别数，$|\gC|$为category的个数)。通过这样的设计，二维矩阵可以用来抽取有关联的aspect和opinion对，且能从标签中直接解码得到它们的category和sentiment。

结果如Tabel~\ref{exp:interaction_result}所示, 除了在Restaurant-ACOS数据集上，在其它三个数据中，我们提出的One-ASQP效果都是最好的，猜测的原因是One-ASQP相比于变种1拆分成三个子任务，One-ASQP的AOSC任务通过sentiment-specific horns tagging schema把aspect、opinion、sentiment捆绑在一起，能让三者充分交互，避免冗余信息。变种2效果是最差的，理论上讲，变种2能使四元素捆绑在一起，但二维矩阵标签空间太大，导致模型学习效率低，模型学习难度大，导致效果不佳。
\end{CJK*}
}

\begin{table}[]
\small
\centering
\begin{tabular}{llclclcl}
\hline
\multicolumn{2}{c}{} & \multicolumn{2}{c}{Variants1} & \multicolumn{2}{c}{Variants2} & \multicolumn{2}{c}{our} \\ \hline
\multicolumn{2}{l}{\textbf{Restaurant-ACOS}} & \multicolumn{2}{c}{\textbf{54.39}} & \multicolumn{2}{c}{49.21} & \multicolumn{2}{c}{54.05} \\
\multicolumn{2}{l}{\textbf{Laptop-ACOS}} & \multicolumn{2}{c}{41.05} & \multicolumn{2}{c}{39.12} & \multicolumn{2}{c}{\textbf{41.70}} \\
\multicolumn{2}{l}{\textbf{en-Phone}} & \multicolumn{2}{c}{38.32} & \multicolumn{2}{c}{36.70} & \multicolumn{2}{c}{\textbf{38.74}} \\ 
\multicolumn{2}{l}{\textbf{cn-FoodBeverage}} & \multicolumn{2}{c}{47.47} & \multicolumn{2}{c}{46.01} & \multicolumn{2}{c}{\textbf{48.07}} \\ \hline 
\end{tabular}
\caption{Result of different element interactions}
\label{exp:interaction_result}
\end{table}
% \end{CJK*}

\subsection{Effect of Negative Sampling}\label{exp:negative_sampling}

\begin{table}[]
\scriptsize
\centering
\begin{tabular}{lccccc}
\hline
\textbf{Mask\_rate} & 0 & \multicolumn{1}{l}{0.2} & \multicolumn{1}{l}{0.4} & \multicolumn{1}{l}{0.6} & \multicolumn{1}{l}{0.8} \\ \hline
\textbf{Restaurant-ACOS} & 43.63 & 46.10 & 48.36 & \textbf{49.29} & 46.87 \\
\textbf{Laptop-ACOS} & 45.32 & \textbf{46.01} & 44.77 & 44.44 & 44.36 \\
\textbf{en-Phone} & 28.49 & 28.63 & \textbf{29.55} & 28.98 & 26.45 \\
\textbf{cn-FoodBeverage} & 38.59 & 36.68 & \textbf{38.71} & 36.53 & 32.35 \\ \hline
\end{tabular}
\caption{Result of Negative Sampling}
\label{exp:negative_sampling}
\end{table}

\blue{
\begin{CJK*}{UTF8}{gbsn}
我们使用网格搜索的方式去研究negative sampling的影响，具体的，我们设定负采样率mask\_rate等于0, 0.2, 0.4, 0.6, 0.8，汇报F1值。如表~\ref{exp:negative_sampling}所示，我们看到不同的数据集有不同的负采样率，大部分在0.4和0.6取得最佳的指标。mask\_rate=0时，所有数据集都取不到最佳的指标，证明了负采样还是必要的。
\end{CJK*}
}
